Chaos in Symmetric Phase Oscillator Networks

Phase-coupled oscillators serve as paradigmatic models of networks of weakly interacting oscillatory units in physics and biology. The order parameter which quantifies synchronization was so far found to be chaotic only in systems with inhomogeneities. Here we show that even symmetric systems of identical oscillators may not only exhibit chaotic dynamics, but also chaotically fluctuating order parameters. Our findings imply that neither inhomogeneities nor amplitude variations are necessary to obtain chaos, i.e., nonlinear interactions of phases give rise to the necessary instabilities.

==> submit 2/commands.tex <==
% CUSTOM COMMANDS AND THEOREMS (in separate file?)


% Theorems etc.

\newtheorem{thm}{Theorem}
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}

%\theoremstyle{definition}
\newtheorem{defn}{Definition}

%\theoremstyle{remark}
%\newtheorem{rem}[thm]{Remark}
%\newtheorem{ex}[thm]{Example}

%\setlength{\theorempreskipamount}{10pt plus 1pt minus 1pt}
%\setlength{\theorempostskipamount}{8pt plus 1pt minus 1pt}
%\setlength{\bigskipamount}{10pt plus 2pt minus 2pt}
%\setlength{\medskipamount}{5pt plus 1pt minus 1pt}
%\setlength{\parskip}{10pt plus 1pt minus 1pt}
%\parindent 0 in

% Enumeration style (1), (2) etc.

%\renewcommand{\labelenumi}{(\arabic{enumi})}
%\renewcommand{\labelitemi}{$\diamond$}
\newcommand{\fref}[1]{(F\ref{#1})}
\newcommand{\headerformat}[1]{\textsc{#1}}
\newcommand{\thmheader}[1]{{#1}}
\newcommand{\lightthmheader}[1]{{\rm #1}}

% Set Symbols

\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\Cc}{\mathcal{C}}

% Math operators
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\Rep}{Re}
\DeclareMathOperator{\id}{id}


% Abbreviations for convenience

\newcommand{\Sym}[1]{S_{#1}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\si}[1]{\sigma_{i_{#1}}}
\newcommand{\s}{\sigma}
\newcommand{\ri}[2]{\varrho_{i_{#1}i_{#2}}}
\newcommand{\rh}{\varrho}
\renewcommand{\th}{\theta}
\newcommand{\rset}[2]{\left\lbrace #1\ \left|\ #2\right.\right\rbrace}
\newcommand{\lset}[2]{\left\lbrace\left. #1\ \right|\ #2\right\rbrace}
\newcommand{\set}[2]{\rset{#1}{#2}}
\newcommand{\sset}[1]{\left\lbrace #1\right\rbrace}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\ci}{\inv{c}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ph}{\varphi}
\newcommand{\G}{\Gamma}
\newcommand{\Rho}{P}
\newcommand{\io}{\iota}
\renewcommand{\Re}{\Rep}
\newcommand{\ind}[1]{_{\mathrm{#1}}}
\newcommand{\vphi}{\varphi}

